Enhancing Reverse Engineering: Investigating and Benchmarking Large Language Models for Vulnerability Analysis in Decompiled Binaries

Security experts reverse engineer (decompile) binary code to identify critical security vulnerabilities. The limited access to source code in vital systems - such as firmware, drivers, and proprietary software used in Critical Infrastructures (CI) - makes this analysis even more crucial on the binary level. Even with available source code, a semantic gap persists after compilation between the source and the binary code executed by the processor. This gap may hinder the detection of vulnerabilities in source code. That being said, current research on Large Language Models (LLMs) overlooks the significance of decompiled binaries in this area by focusing solely on source code. In this work, we are the first to empirically uncover the substantial semantic limitations of state-of-the-art LLMs when it comes to analyzing vulnerabilities in decompiled binaries, largely due to the absence of relevant datasets. To bridge the gap, we introduce DeBinVul, a novel decompiled binary code vulnerability dataset. Our dataset is multi-architecture and multi-optimization, focusing on C/C++ due to their wide usage in CI and association with numerous vulnerabilities. Specifically, we curate 150,872 samples of vulnerable and non-vulnerable decompiled binary code for the task of (i) identifying; (ii) classifying; (iii) describing vulnerabilities; and (iv) recovering function names in the domain of decompiled binaries. Subsequently, we fine-tune state-of-the-art LLMs using DeBinVul and report on a performance increase of 19%, 24%, and 21% in the capabilities of CodeLlama, Llama3, and CodeGen2 respectively, in detecting binary code vulnerabilities. Additionally, using DeBinVul, we report a high performance of 80-90% on the vulnerability classification task. Furthermore, we report improved performance in function name recovery and vulnerability description tasks.

==> sections/10_ethics.tex <==
The purpose of this paper is to further advance cyber security research with large language models. Code vulnerabilities can cause significant damage to individuals and organizations. For this reason, we have decided to not make publicly available our prompting techniques and source code for injecting vulnerabilities into clones of open-source repositories.

==> sections/2_background_and_motivation.tex <==


\subsection{Problem Definition}
We define the textual summary of decompiled function $\mathcal{F}$ as $S$, which is an accurate human-readable summary of the semantics of $\mathcal{F}$. We then define the code summarization task as function $\beta$ where $\mathcal{F}$ is summarized as $S$:
\begin{center}
    $S = \beta(\mathcal{F})$ \quad (1)
\end{center}
The binary classification task of whether $S$ contains text describing a vulnerability is denoted by $V$. To determine this, we define another function $\Gamma$ that determines if vulnerability indicators, such as keywords and phrases, are present in $S$
\begin{center}
    \begin{align}
    \mathrm{\Gamma}(x) = \begin{cases}
        1 & \text{if } x \text{ contains vulnerability indicators} \\
        0 & \text{otherwise}
    \end{cases}
    \end{align}
    $V = \Gamma(S)$ \quad (2)
\end{center}
If $V > 0$, then $S$ is a summary that contains text describing a vulnerability. Otherwise, $S$ is a summary that does not consider vulnerabilities.

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figures/re_process.png}
    \caption{The process of compiling source code and decompiling binaries.}
    \label{fig:decompile_process}
\end{figure*}

\subsection{Challenges in Decompiled Binaries}
\label{sec:challenges}
Reverse engineers face many challenges when analyzing decompiled code. Understanding the objective and semantics (i.e., the summary $S$) of decompiled code is generally more complex than understanding the semantics of source code. During the decompilation process, the variables or the flow of statements sometimes get changed for optimization. As a result, working with decompiled code for tasks such as vulnerability analysis or decompiled code summarization \cite{al2023extending} is more challenging. Specifically, we discuss five challenges faced with decompiled code for summarization tasks.


\paragraph{\textbf{C1: Comments do not Exist}} When source code is compiled, comments are typically ignored by the compiler and no longer exist in the compiled binary. Therefore, comments are irrecoverable in decompiled code. Without comments, comprehending decompiled code is incredibly challenging and time-consuming as it provides limited information about its purpose and intended behavior. Therefore, the reverse engineer has to derive meaning from syntax and structure. This issue is observed in Figure \ref{fig:decompile_process} where the \textit{"Do not append the empty string"} comment in line 2 is removed from the \texttt{jsonAppendRaw} function during compilation and, therefore, cannot be recovered in the decompiled \texttt{jsonAppendRaw} function.


\paragraph{\textbf{C2: Misleading Function Calls}} When source code is compiled, the compiler may optimize the code by replacing common function calls, such as \texttt{strcpy}, with a custom function that performs the same task more efficiently. Alternatively, the compiler may optimize the binary by inlining the instructions of common function calls in the callee function, effectively removing the function call altogether. This may prove challenging for reverse engineers who are attempting to identify code semantics through commonly called functions. This phenomenon is exemplified in Figure \ref{fig:decompile_process}, where the unsafe standard C library function, \texttt{memcpy}, is replaced with \texttt{func\_0x00111e30} in the decompiled code. This usually happens during decompilation since the dissembler does not know the original function name and the replaced string \texttt{func\_0x00111e30} is the address of the function in the system memory. 


% When a disassembler encounters a call to the memcpy() function, it will typically convert it to a call to a function with a name like func_0x00111e30. This is because the disassembler does not know the original name of the function. The number 0x00111e30 is the address of the function in memory.

%\textcolor{red}{Bit overuse of the term reverse engineer}

\paragraph{\textbf{C3: Complex Control Flow}} The control flow of the source code may be optimized and modified in the compiled binary. As a result, the decompiled code may have a more complex control flow of statements, which is difficult to understand from a reverse engineer's perspective. A common example is loop unrolling \cite{sarkar2000optimized, huang1999generalized}, where a loop is unraveled as a sequence of instructions instead of jumping back to the beginning of the loop until a condition is met. However, these optimizations can sometimes be unusual and confusing when comprehending the flow of decompiled code. In Figure \ref{fig:decompile_process}, we see the body code of the \texttt{if-else} blocks were swapped, and the expression \texttt{N==0} (or \texttt{param\_3==0} in decompiled code) was inverted to \texttt{N!=0} or (or \texttt{param\_3!=0} in decompiled code). As a result, while the decompiled code maintains similar functionality, the readability of the code is vastly reduced.

\paragraph{\textbf{C4: Variable Type Obfuscation}} The compilation process can strip away type information, or the decompilation process may misrepresent type information (such as a pointer becoming a \texttt{long}). This may be done to compress binary size or to obfuscate code. Although prior work in decompilation focuses heavily on recovering types \cite{chen2020cati,lehmann2022finding}, type inference is not always accurate. Having unknown or incorrect types of variables may make it challenging for reverse engineers to understand the semantic meaning of the decompiled code. An example of this can be seen in Figure \ref{fig:decompile_process} where the source code type of \texttt{JsonString *} was inferred as \texttt{long}, the source code type \texttt{char *} was inferred as \texttt{undefined8}, and the source code type \texttt{u32} was inferred as \texttt{uint}.

\paragraph{\textbf{C5: Variable Names Obfuscation}} Similar to \textbf{C4}, The compilation process can remove variable names. Additionally, some software developers use obfuscation techniques by renaming their variables to ambiguous names to make their code more difficult to decompile deliberately for prote action of their code \textcolor{red}{Need Citation} \cite{BEHERA2015757}. Variable names play a crucial role in understanding the meaning and intent of code by providing a clear and concise way to represent the variable's purpose. While prior work in decompilation exists on recovering variable names \cite{kim2023transformer,lacomis2019dire}, it is not always accurate. Without representative variable names, reverse engineers must infer the identity of the variable, hindering the understanding of the decompiled code's semantics. This is observed in the decompiled code of Figure \ref{fig:decompile_process}, where the parameter names are all generic such as \texttt{param\_1}, \texttt{param\_2}, and \texttt{param\_3}, and do not provide any information regarding the intent of these variables.

%\subsection{Motivation}
%The code summarization task is a recent development in large language model research \cite{zhang2022survey} primarily for documentation purposes. This helps both software engineers and reverse engineers to better understand and comprehend function semantics. However, as shown in Table \ref{tab:related_work_comparison}, previous works have failed to mention vulnerability detection for reverse engineers as an result of their work. Summarizing decompiled functions with vulnerability-awareness has the potential for This limitation directly motivates us to propose \texttt{REDVulLLaMA}.

==> sections/3_investigation.tex <==

% Investigation goal is to show the semantic gap

% Good

%This section introduces a vulnerable code injection attack to demonstrate semantic changes in binary code, which can negatively impact the performance of LLMs in analyzing such code.
% In this section, we are the first to empirically and pragmatically investigate the analytical abilities of \textit{state-of-the-art} black-box LLMs in analyzing vulnerabilities in the decompiled binary code domain. While previous studies, such as \cite{islam2023unbiased}, \cite{wang2024combining}, and \cite{liu2024source}, have shown significant advancements in vulnerability analysis using transformer-based LLMs on static source code, their effectiveness on decompiled binary code remains uncertain. \textit{An illustrative figure of our investigation pipeline is provided in Appendix; Figure \ref{fig:investigation}}.\\


% functions functions from our proposed dataset, and then compiled and decompiled them with Ghidra. The two variants, static source code and decompiled binaries were used as input for the LLMs to assess their capability in identifying and classifying these vulnerabilities. Further details on the data and methodology are provided in Section \ref{qa4binvul} \textit{Data Collection}, and the investigation process is illustrated in Figure \ref{fig:investigation}.


%In this section, we introduce a vulnerable code injection attack, using a part of our proposed dataset to establish the existence of semantic change in binary code, which, in turn, diminishes the performance of LLMs when analyzing binary code. Previous works like \cite{islam2023unbiased}, \cite{wang2024combining}, and \cite{liu2024source} have shown that transformer-based LLMs have shown significant improvement in analyzing vulnerability in static source code. However, it is still unclear from these analyses how binary code would perform with LLMs. Therefore, we investigate the vulnerability identification and classification capabilities of LLMs in binary code. In order to perform this analysis, we extracted functions from real-world repositories, injected vulnerabilities with LLMs, and compiled and decompiled them using Ghidra. Since we injected vulnerabilities in the functions of the original source code, the decompiled binaries are also infected with vulnerabilities. We used this decompiled code as input for the LLMs to identify and classify vulnerabilities. The details of the data used for investigation are described in \ref{qa4binvul} \textit{Data Collection}, and the flow of the investigation is demonstrated in Figure \ref{fig:investigation}.

% Cite other papers on comparing src code vs decom. binaries performance

%the effectiveness of publicly available state-of-the-art (SOTA) large language models in analyzing vulnerability in decompiled code. Our analysis includes identifying, classifying, and describing the decompiled code. We aim to analyze vulnerability in decompiled code by injecting vulnerability in the source code. Then, we assess how effectively and accurately these LLMs can analyze vulnerabilities in decompiled code in a zero-shot setting. However, we found no existing dataset specifically tailored for analyzing the security aspects of decompiled code. Therefore, we generated vulnerability-injected code consisting of real-world repositories. 

%Our experiment consists of using heavily used general-purpose and code-purpose LLMs. In the following subsections, we explain in detail how we injected vulnerabilities in code from real-world repositories and empirically evaluate how they perform on SOTA LLMs including API-based access and open-access models. Figure \ref{fig:investigation} shows the overall pipeline of code injection in repositories and analyzing them using SOTA LLMs. 




%\subsection{Preliminary Background}
% Nafis: Intentionally Removing Paragraph
% \paragraph{\textbf{Binary Vulnerability Analysis}} 
% Code vulnerability could be assessed by analyzing static or binary source code \cite{islam2023unbiased, sejfia2024toward, islam2024code, luo2023vulhawk}. However, the extensive use of C/C++ programs in legacy software like Linux Kernel makes them susceptible to vulnerability. Analyzing vulnerability in legacy software becomes even more challenging when it is closed-source, making it impossible to access the source code. Thus, decompiled binary vulnerability analysis \cite{luo2023vulhawk,li2023vulanalyzer} is a more viable option \cite{yu2023cfg2vec}. 

%Since C/C++ allows direct manipulation of memory and hardware resources and provides a higher level of control, it can potentially introduce vulnerabilities such as buffer overflows, pointer arithmetic errors, and memory corruption. With automatic garbage collection, C/C++ requires programmers to manage memory manually. This manual management increases the risk of memory leaks, dangling pointers, and other memory-related vulnerabilities, making these languages more prone to specific security issues.



% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}



%(Think again)Furthermore, for legacy software, it is possible that the original source code, developers, and support may no longer exist, making binary vulnerability analysis a more suitable approach \cite{yu2023cfg2vec}.

% DO NOT DELETE THESE FOLLOWING PARAGRAPHS: THEY WILL GO TO DATASET SECTION
%------------------------------------------------------------------------%

%\textcolor{red}{Move to Experiments: Compilation and Decompilation}
%\paragraph{\textbf{Compilation and Decompilation}} Software compilation is a complex process that involves translating source code written in a high-level programming language into machine code that can be executed by a computer. This process includes several stages, such as preprocessing, compiling, assembling, and linking, which work together to generate a compiled binary. In contrast, decompilation is the inverse process of converting a binary into high-level source code. This complicated process requires a reverse engineering tool such as IDA Pro \footnote{https://hex-rays.com/ida-pro/}, Ghidra \footnote{https://ghidra-sre.org/}, or Angr \footnote{https://angr.io/} that first disassembles the binary into low-level intermediate assembly code. Finally, the reverse engineering tool uses a decompiler to lift the low-level intermediate assembly code into high-level pseudo-source code.














%%%%%%%%%%%%%%%%%







%\paragraph{\textbf{Vulnerability Injection and Description Build Process}} 



%Out of the 37 samples, we reverted 32 samples to the original function and removed them from our red team data and the remaining 5 samples were fixed manually and were kept in the dataset. We manually addressed the minor errors by correcting the fields (variable names or functions) referenced in the generated code, calling the correct functions, and fixing syntax errors, but not patching the vulnerability. 


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[t]
\centering
\caption{LLMs semantic gap comparison between static source code and decompiled binary code on vulnerability classification task. Reported average F1-scores.}
\begin{tabular}{@{}llll@{}}
\toprule \toprule
\textbf{Input Type} & \textbf{GPT4}    & \textbf{Gemini}  & \textbf{CodeLLaMa} \\ \midrule \midrule
\textbf{Source Code}     & 0.75            & 0.68             & 0.64               \\
\textbf{Dec. Binary Code} & 0.67 \textcolor{red}{$\downarrow$}            & 0.54 \textcolor{red}{$\downarrow$}            & 0.54 \textcolor{red}{$\downarrow$}              \\\\ \midrule\midrule 
                    & \textbf{Mistral} & \textbf{LLaMa 3} & \textbf{CodeGen2}  \\ \midrule \midrule
\textbf{Source Code}     & 0.60             & 0.45             & 0.64               \\
\textbf{Dec. Binary Code} & 0.54 \textcolor{red}{$\downarrow$}            & 0.33 \textcolor{red}{$\downarrow$}            & 0.52 \textcolor{red}{$\downarrow$}              \\ \bottomrule
\end{tabular}
\end{table}

% \subsection{Investigation Setup.}
% % Show the numbers for decompiled code for CodeLLaMA%
% \label{sec:decomp_investigation}


%With our decompiled vulnerable code, we tasked \texttt{ChatGPT-4} \cite{OpenAI2023GPT4}, \texttt{Gemini} \cite{Google2023Gemini} and \texttt{CodeLLaMA-7B} \cite{roziere2023code}, Mistral \cite{jiang2023mistral}, LLaMa 3 \cite{touvron2023llama} and CodeGen2 \cite{nijkamp2023codegen2} in identifying and classifying vulnerable both the injected vulnerable and benign decompiled functions. We designed a carefully crafted prompt to use the generative capability of the LLMs to answer “Yes/No” when the prompt was about the existence of the vulnerability. Furthermore, the prompt also enforces the LLM to generate the CWE number of the vulnerability, provided it exists. We want to classify the vulnerability, and the prompt has been changed so that the LLM only outputs the CWE category. Then, based on the outcomes generated by the mentioned LLMs, we formulate and analyze Table \ref{tab:motivation}. The prompts used for these LLMs are available in Appendix \ref{9_appendix} \textit{\textcolor{red}{Prompts and Investigation}}.


In this section, we are the first to empirically and pragmatically investigate the analytical abilities of \textit{state-of-the-art} LLMs in analyzing vulnerabilities in the decompiled binary code domain. To explore this, we randomly select \textit{200} pairs of vulnerable and non-vulnerable source code and decompiled binary code samples from our proposed dataset, \textcolor{VulBinCode}{\textbf{DeBinVul}} \footnote{Please refer to the Proposed Approach Section for details on the dataset.} for the task of classifying vulnerabilities. Specifically, we evaluate the ability of several LLMs, including \texttt{ChatGPT-4} \cite{OpenAI2023GPT4}, \texttt{Gemini} \cite{Google2023Gemini}, \texttt{CodeLLaMA-7B} \cite{roziere2023code}, Mistral \cite{jiang2023mistral}, LLaMa 3 \cite{touvron2023llama}, and CodeGen2 \cite{nijkamp2023codegen2}, to identify and classify vulnerabilities in both source code and decompiled binary code. Table \ref{tab:motivation} presents the comparison results and underscores the semantic vulnerability limitations of \textit{state-of-the-art} black-box LLMs in classifying \texttt{CWEs} in decompiled binary code, in contrast to source code, which presented moderately better results. The reported results in Table \ref{tab:motivation} focuses on \texttt{CWEs:} \texttt{787}, \texttt{416}, \texttt{20}, \texttt{125}, \texttt{476}, \texttt{190}, \texttt{119}, \texttt{798} and reports their average F1-scores. 











A carefully designed prompt was used to leverage the generative capabilities of these LLMs, asking them to respond with a “Yes” or “No” regarding the presence of vulnerabilities. Additionally, the prompt required the LLMs to generate the corresponding CWE number if a vulnerability was detected. To classify the vulnerabilities, the prompt was adjusted to ensure that the LLMs only output the CWE category. The results from these LLMs are summarized and analyzed in Table \ref{tab:motivation}. The specific prompts used in this analysis are provided in Appendix \ref{9_appendix} \textit{\textcolor{black}{Prompts and Investigation}}.




\paragraph{Result Analysis}
The results from Table \ref{tab:motivation} in Appendix show that API-based models like GPT4 could accurately identify a vulnerability in decompiled binaries with an accuracy of 70\%, where Gemini is at 56\%. Moreover, open models like CodeLLaMa is at 61\%, Mistral is at 54\%, LLaMa 3 at 50\%, and CodeGen2 at 54\%.  Moreover, from Table \ref{tab:motivation}, we see that GPT-4 performs comparatively higher overall than other API-based or open-access models. To investigate the details of the identification task, we investigate how accurately these LLMs can classify each vulnerability category. The results show that all models were experts at identifying some vulnerabilities and failing at others. For example, GPT4, Gemini, Mistral, and LLaMa 3 produce higher performance on CWE-416, CodeLLaMa on CWE-20, LLaMa 3 on CWE-190, and CodeGen2 on CWe-476. However, one interesting observation from our analysis is that while CodeLLaMa, Mistral, and CodeGen 2 are moderately successful in identifying vulnerability, these LLMs fail to predict most CWEs. Therefore, we can conclude that CodeLLaMa has a very limited understanding of the vulnerability category. Furthermore, Table \ref{tab:motivation} provides more detailed numerical results, including Accuracy, Precision, Recall, and F1 score. Section \textit{Reasoning of Weak Performance in Investigation} in Appendix \ref{9_appendix} explains the reason behind the poor performance of LLMs when analyzing decompiled binaries. 



%\textcolor{red}{Add few shot}

%% TODO: Added by Joseph






%Another interesting observation is that while CodeLLaMa is a code-based model, its expertise mostly lies in analyzing the functional aspects of source code and not much on security.
%CodeLLaMa could not correctly predict the CWE number of any other vulnerable code. This confirms our initial intuition that CodeLLaMa was inefficient enough to analyze the security aspects of vulnerable code of decompiled binaries.



%Furthermore, if we see the frequency of the predicted classes by GPT-4 in the bar chart in Figure 1, we can see that the frequency of the predicted classes for of different functions by GPT-4 is the highest for CWE-787, and  followed by CWE-416, CWE-119 and CWE-121. This imbalance of frequency further confirms that the model is mostly biased towards CWE-787 and achieved higher accuracy in identifying vulnerable functions by predicting majority of functions as vulnerable and classifying them as CWE-787.






% \paragraph{\textbf{Comments}} Unless the compiler has debug information available, it is impossible for these models to address \textbf{C1} because comments will not be present in the decompiled code. Comments play a large role in source code summarization because there is usually a correlation between the type of comment associated with a code block and the functionality or purpose of the code block itself, where some comments describe how the code works and others explain the reasoning behind certain design choices \cite{chen2021my}. Additionally, some software developers will annotate potential bugs in their code with \texttt{FIXME} comments, which may help in describing vulnerabilities in code summarizations \cite{phaithoon2021fixme}.

% \paragraph{\textbf{Types and Names}} As many prior works in reverse engineering focus on recovering lost information in decompiled code \cite{chen2020cati,lehmann2022finding,kim2023transformer,lacomis2019dire}, \textbf{C2}, \textbf{C4}, and \textbf{C5} can be mitigated. However, to the best of our knowledge, these models do not implement these mechanisms.

% \subsection{Vulnerability Summarization}

% We aim to answer the following question here:

% \textit{Are open-source LLMs capable of understanding and describing vulnerable and non-vulnerable decompiled code?}

% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% \begin{table}[b]
% \centering
% \caption{Performance of Describing the Objective of a and Security Description of a Vulnerable Function. We used Semantic metrics like BERTSCore and Syntactic Metrics Like BLEU, Rouge-L, Meteor, and also Human Evaluation (HE)}
% \begin{tabular}{@{}llllll@{}}
% \toprule
% \textbf{Model} & \textbf{BERTScore} & \textbf{Rouge-L} & \textbf{BLEU} & \textbf{METEOR} & \textbf{HE} \\ \midrule
% GPT-4          & 0.82      & 0.20             & 0.04          & 0.24            &                           \\
% Gemini         & 0.83      & 0.20             & 0.04          & 0.20            &                           \\
% CodeLLaMa      & 0.83      & 0.21             & 0.04          & 0.25            & \\  

% BinT5      & 0.83      & 0.21             & 0.04          & 0.25            & 
% \\ \bottomrule
% \end{tabular}
% \label{tab:moti_summary}
% \end{table}

% We ran an experiment to determine how well GPT4, Gemini, and CodeLLaMa understood and generated descriptions for decompiled code. Again, we used the same decompiled code from the previous section and the ground truth description generated by GPT-4.




% %\paragraph{Result Analysis:} 

% We calculated BERTScore, Rouge-L, BLEU, METEOR, and Semantic Similarity to evaluate the generated code descriptions. Moreover, we used human evaluation as a sanity check for automated methods of generated descriptions. Table \ref{tab:moti_summary} shows that all the scores closely match every metric. However, CodeLLaMa has a slightly improved BERTScore over Gemini and GPT-4. To understand the vulnerabilities, we present a qualitative analysis of the generated decompiled code descriptions. From Listing \ref{lst:lst1}, we see that, when working with decompiled code, GPT-4 produced descriptions that, while still accurate, tended to be more vague about the specific purpose of the code. This vagueness is likely due to the inherent loss of information during the decompilation process, which makes the code less readable and more challenging to interpret. However, from the generated outcome of Gemini, we see that the code description is very short but slightly more specific compared to GPT-4. Finally, we found that CodeLLaMa generates the most distinctive and clear flow of description of the code compared to the other two LLMs.

%% May bring back later
%Our analysis indicates that GPT-4 and Gemini outperform CodeLLaMa and other models for vulnerability identification in decompiled code. Although CodeLLaMa excels over Gemini in identifying vulnerabilities, it significantly underperforms in classification tasks. Conversely, CodeLLaMa demonstrates superior capability in describing the objectives and vulnerabilities of decompiled code. However, none of the models consistently excels across all tasks required for comprehensive vulnerability analysis in decompiled code. Therefore, our work aims to provide a single LLM that excels at these tasks and analyzes vulnerabilities.



%From our analysis, we can see that while closed-source models perform relatively better, open-source models like CodeLLaMa have a very poor understanding of the vulnerability of decompiled source code. However, we also notice that CodeLLaMa has a very good understanding of the objective of a decompiled binary.


==> sections/6_case_studies.tex <==
To demonstrate how one can use \texttt{REDVulLLaMA} in real-world applications, we present two use-cases. The first application \textcolor{red}{TODO: app}. The second application \textcolor{red}{TODO: app}. We discuss each application in the following subsections.

==> sections/7_limitations.tex <==
This section describes the limitations of our work and future considerations.

\paragraph{\textbf{Other Compiler Considerations}} \texttt{REDVulLLaMA} is only trained on unstripped decompiled code that was compiled at the \texttt{O2} optimization level for \texttt{gcc}. The results of \texttt{REDVulLLaMA} may be different on various compilers and different optimizations levels which can modify the underlying binary. Additionally, the scope of our work only encompasses Linux x86-64 binaries, and does not cover other operating systems or architectures.

\paragraph{\textbf{Languages}} \texttt{REDVulLLaMA} is only trained and evaluated on decompiled C/C++ code. Our model and InstructDecomp does not consider other compiled languages such as Rust or Go.

\paragraph{\textbf{Obfuscation}} To the best of our knowledge, \texttt{REDVulLLaMA} was not trained on obfuscated samples. Additionally, none of the compiled binaries were encrypted or packed. The decompiled code may vary significantly and affect the results of \texttt{REDVulLLaMA} with these considerations in mind.

\paragraph{\textbf{Dataset Size}} We only train and evaluate \texttt{REDVulLLaMA} on a small portion of our dataset. While our dataset is large, it only contains decompiled code of two repositories. A dataset that encompasses more diverse open-source repositories may improve the performance of \texttt{REDVulLLaMA}.
